Multi-Sentence Resampling: A Simple Approach to Alleviate Dataset Length Bias and Beam-Search Degradation

Neural Machine Translation (NMT) is known to suffer from a beam-search problem: after a certain point, increasing beam size causes an overall drop in translation quality. This effect is especially pronounced for long sentences. While much work was done analyzing this phenomenon, primarily for autoregressive NMT models, there is still no consensus on its underlying cause. In this work, we analyze errors that cause major quality degradation with large beams in NMT and Automatic Speech Recognition (ASR). We show that a factor that strongly contributes to the quality degradation with large beams is \textit{dataset length-bias} - \textit{NMT datasets are strongly biased towards short sentences}. To mitigate this issue, we propose a new data augmentation technique -- \textit{Multi-Sentence Resampling (MSR)}. This technique extends the training examples by concatenating several sentences from the original dataset to make a long training example. We demonstrate that MSR significantly reduces degradation with growing beam size and improves final translation quality on the IWSTL$15$ En-Vi, IWSTL$17$ En-Fr, and WMT$14$ En-De datasets.

==> related_work.tex <==
\section{Related Work}

%\todo{Speak about methods don't mentioned in Introduction, about context research, problems with not-in-train lengths in transformers... Concerning context it is interesting to test how our method will behave on Context tasks}

An interesting line of research study calibration properties of Neural Machine Translation. Calibration measures how much the generated by the model distribution matches the actual data distribution. As shown in~\citep{calibration-of-encoder-decoder}, NMT architectures are poorly calibrated. EOS token is the worst calibrated, and tokens with high entropy of attention weights are also worse calibrated than others. \citep{inference-calib-2020} found that high-frequency tokens are less likely to be poorly calibrated, while low-frequency tokens often suffer from miscalibration. Our work shows that underrepresented lengths contribute to quality degradation with large beam sizes and that degradation mainly comes from early appearing EOS tokens, which support the results of the calibration studies.

~\citep{breaking-beam-curse-2019} analyzed rescoring and reward methods for beam-search. ~\citep{predicting-length-2020} proposes to predict and use target length during decoding. In contrast, our work does not change the search procedure, instead of this we show that augmenting the train dataset with \textit{Multi-Sentence Resampling} can mitigate beam search degradation with large beams.

%The idea of encouraging long sentences with additional rewards is adjacent to Reinforcement Learning methods that try to learn sequence-level objectives in NMT~\citep{ranzato2016sequence, study-rl-for-nmt-2018, Wu2016GooglesNM, seq-pred-with-reward, bahdanau2017actorcritic}, and to similar minimum risk training~\citep{minimum-risk-training}.

%\citep{beam-search-question} shows that beam-search enforces uniform information density across the output and proposes making this property more effective. \citep{map-decoding-all-you-need} shows that after small amount of samples in-domain, the model covers almost all probability space, while the opposite picture is out-of-domain. ~\citep{wang-sennrich-exposure-2020} study properties of NMT generation procedure under domain shift.

%A close domain to our work is Context-Aware Machine Translation~\citep{nmt-with-extended-context-2-2017, exploiting-cross-sentence-chinese-2017, voita-etal-2018-context, document-memory-2018, voita-etal-2019-good}. These papers analyze how context information can help in NMT. They use datasets where adjacent sentences are meaningfully connected, opposite to \textit{Multi-Sentence Resampling} that uses independent sentences.

%\section{Future Research}
%It is interesting to adapt \textit{Multi-Sentence Resamling} to ASR. This is harder than in NMT, as the input signal is more complex. Another interesting point is the behavior of beam-search problem and length bias in Context-Aware Machine Translation. Our paper suggests that beam-search problem can be mitigated if using several sentences. However, to the best of our knowledge, there is no research that study beam-search problem in this domain. 


%Most popular architectures that generate language are autoregressive \cite{Attentionallyouneed}, be it neural machine translation, language generation or dialogue systems. During decoding these models give higher probability for shorter sequences than for longer sequences. This well-known problem is called \textbf{Length bias}. 

%In~\citep{2016-length-bias} it was shown that training-loss of the encoder-decoder model underestimates the margin of separating long sequences from short ones. It was also mentioned that when there is a high entropy of our local distribution, for example, many equally probable continuations of the sentence (synonyms), the \textbf{length bias} will be even worse because the probability of the long sequences will decrease faster. In~\citep{cat-tongue} it was shown that exact search by likelihood for neural machine translation finds empty string as the optimal hypothesis in more than $50 \%$ of cases. This problem is the property of the current probability space that modern architectures learn. It causes a dramatic drop in the quality of translation for long sentences~\citep{mt-problems-2017}.


%On top of the trained autoregressive model REINFORCE algorithm was used to optimize BLEU or ROGUE. However, ~\citep{Wu2016GooglesNM} shows that while Reinforcement Learning helps to improve BLEU score, this improvement does not reflect human-evaluation scores. This is because BLEU is not a direct assessment of the translation quality, but only its approximation.

%One of the famous consequences of \textbf{length bias} is the decreasing quality of beam-search with larger beams, or \textbf{beam-search problem}. With growing beam size, beam-search finds more and more likely and shorter, but not correct hypotheses. In~\citep{breaking-beam-curse-2019}, larger beams beam-search generates EOS earlier and dramatically drops BLEU score. In this work, it was proposed to use several rescoring techniques that change scores during decoding. These techniques add rewards for each generated word in beam-search, thus encouraging longer sentences. They first learn a separate model to predict the length of the generated sentence and then provide rewards to the model based on it. This alleviates decreasing scores with larger beam-sizes and increases BLEU for larger sentences. Another bunch of techniques that are trying to change scores in beam-search in order to solve \textbf{beam-search problem} is popular \textit{length normalization} technique~\citep{bahdanau2016neural, Wu2016GooglesNM} that basically use an averaged over tokens in a sentence score to compare hypotheses in the beam. Although in these papers it was suggested to change beam-search scoring procedure by adding rewards or normalizing scores by length, these methods do not try to solve the source of \textbf{beam-search problem} that is in \textbf{bad likelihood approximations produced by the model} for sentences. The property that makes probability predictions of the model for shorter sentences inadequately higher than for long sentences.

%The idea of encouraging long sentences with additional rewards is adjacent to Reinforcement Learning methods. In~\citep{ranzato2016sequence} it was proposed to use Reinforcement Learning for sentence-level score optimization. On top of the trained autoregressive model REINFORCE algorithm was used to optimize BLEU or ROGUE. However, ~\citep{Wu2016GooglesNM} shows that while Reinforcement Learning helps to improve BLEU score, this improvement does not reflect human-evaluation scores. This is because BLEU is not a direct assessment of the translation quality, but only its approximation.

%Another exciting line of research tries to improve Natural Language Generation by allowing the model to generate tokens in arbitrary order~\citep{gu-etal-2019-insertion, non-monotonic-generation, dmitrii-unc-gen-ord, XLNet}. This allows the model to choose in what order to generate output sequence and increase decoding quality. In~\citep{gu-etal-2019-insertion} the Transformer model predicts not only a word at each step but also its relative position to already generated words. This work improves generation quality and shows that with such architecture, the quality of the generated sequence grows with growing beam size. Based on this work, we can say that such methods of allowing a model to generate text in arbitrary order help solve \textbf{beam search problem}. Also, we can assume that such methods improve the quality of probability distribution over generated sequences. \textit{However, no one yet researched this question.} Even for beam search, there are only experiments until the beam size of 20. (Dima said that they had not got a decrease in quality until beam size of 128, however it is not published. Further sizes are not explored). Also, it is worth to mention that such models are significantly slower during training (up to 8 times).

%Discussed problems can be seen as calibration problems. It was recently shown that predictions of modern neural networks are often poorly calibrated~\citep{on-calib-of-modern-nn}. Calibration is crucial in all cases where the approximate search is used. Such as machine translation, where the resulting score is a product of many local scores. Increasing the beam size almost always outputs a higher scoring prefix, but if the score is not calibrated, that does not guarantee more correct outputs. The more prefixes we have with over-confident scores, the higher is our chance of over-shadowing the true best prefix in the next step, causing accuracy to drop with increasing beam-size. As shown in~\citep{calibration-of-encoder-decoder} neural machine translation architectures are very poorly calibrated, even they are conditioned on previous true tokens. They also showed that the EOS token is the worst calibrated, and tokens with high entropy of attention weights are also worse calibrated than others. In~\citep{inference-calib-2020} several interesting facts were shown. They found that high-frequency tokens are less likely to be poorly calibrated, while low-frequency tokens often suffer from miscalibration. It was also shown that decoder size negatively affects calibration, while Label smoothing and Dropout improve calibration. Label smoothing greatly reduces over-estimation at the cost of increasing the percentage of under-estimation error. In~\citep{map-decoding-all-you-need} it was shown that while label-smooting improves calibration of the model, it is very hard to distill a teacher network trained with label smoothing. While such teachers' quality is better than a network trained without label smoothing, the picture is the opposite after distillation. Label smoothing encourages examples to lie in tight, equally separated clusters, so every example of one class has very similar proximities to examples of the other classes. Therefore, a teacher with better accuracy is not necessarily the one that distills better.

%In~\citep{beam-search-question} the authors show that beam-search works good because it enforces \textbf{Uniform information density}. The UID hypothesis states that—subject to the grammar constraints—humans prefer sentences that distribute information (in the sense of information theory) equally across the linguistic signal, e.g., a sentence. Several regularizers to enforce this property were introduced in this paper. In general, all of them are trying to make scores obtained by beam-search for tokens at each step more uniform. They significantly reduce the drop of accuracy with larger beam sizes; however, there is no increase in accuracy with larger beams. 


%In~\citep{map-decoding-all-you-need} the authors performed an analysis of MAP decoding. They showed that after 1000 samples in-domain the model covers almost all probability space, while out-of-domain only small part of it. They also test Minimum Bayes Risk scoring with sampling and show that you can achieve beam-search using it. Minimum Risk methods were also used in other papers~\citep{minimum-risk-training, nmt-by-minimizing-risk}.


%Autoregressive Automatic Speech Recognition~\cite{fairseq-s2t,Mohammed-arxiv} is the field very similar to the neural machine translation. And autoregressive models suffer from the same bunch of problems.

%In~\citep{renormalize-prob-pruning-beam-asr} authors showed that ASR systems suffer from beam search problem, however drop in quality seems to grow very slowly with beam size, and simple heuristics like length normalization eliminate this problem with even large beam sizes. Also, in this article authors proposed to explicitly renormalize probability of hypotheses ended in some position to all hypotheses that ended in this position, however this probabilities are very hard too compute, so authors used pruned beam search to approximate such probabilities. Their method seems to eliminate the problem even in 5000 beam size for a ASR model. Still they use heuristic and do not clarify why and through what channel this quality drop comes.

%In general there is much less research of our problems of interest for ASR models compared to NMT.
